Comparative analysis of structural, elastic, electronic, phonon, thermal and optical properties of two $\text{Na}_6\text{Ge}_2\text{Se}_6$ phases from first principles calculations

The demand for new alkali metal chalcogenide materials is continuously increasing due to their potential applications across various technological fields. Recently, a new compound, $\text{Na}_6\text{Ge}_2\text{Se}_6$, was computationally predicted, representing a new phase distinct from the experimentally observed $\text{Na}_6\text{Ge}_2\text{Se}_6$ reported in 1985. Notably, this newly predicted phase displays a lower total energy compared to the previously known experimental phase, as determined by first-principles calculations. In this study, we undertake a thorough comparative analysis of the structural, elastic, electronic, phonon, thermal, and optical properties of these two $\text{Na}_6\text{Ge}_2\text{Se}_6$ phases. Our results show that both phases meet mechanical and dynamical stability criteria. The electronic band structure analysis confirms the semiconducting nature of both materials, with a 2.97 eV indirect band gap for the predicted phase and a 2.93 eV direct band gap for the observed phase. Optically, both phases exhibit strong absorption in the ultraviolet region. Thermal properties analysis reveals that the predicted phase is more thermodynamically stable below 907 K, while the observed phase shows greater thermodynamic stability above this temperature.

==> draft.tex <==
Theoretical calculations for both NaGeSe phases based on first principles, including band structure (BS), partial and total density of states (PDOS, TDOS) have been performed, as shown in Fig. 4. In the BS spectrum, both NaGeSe phase shown to be an direct band gap compound with a calculated band gap of 1.873 eV for observed NaGeSe phase with the bottom of the conduction band (CB) and the top of the valence band (VB) are located at the Y2 point. and 1.832 eV for predicted NaGeSe phase with CB and VB at the M point. The PDOS and TDOS calculations show that, for both NaGeSe phases the region near the Fermi level is mainly composed of Se p and Ge 4p and 4s states while Se 4s orbital takes a minority part near the Fermi level It implies that the band gaps of both NaGeSe phases are mainly determined by the [Ge2Se6] dimers. In the valence band from −5 to 0 eV, Ge 4s, 4p and Se 4s orbitals are the main contributions, and the same circumstance happens at the bottom of the conduction band. Besides, Na makes a small contribution to the bottom of the conduction band from 0 to 7 eV, as shown in Fig.5


